Uncertainty-aware Self-training for Text Classification with Few Labels

Recent success of large-scale pre-trained language models crucially hinge on fine-tuning them on large amounts of labeled data for the downstream task, that are typically expensive to acquire. In this work, we study self-training as one of the earliest semi-supervised learning approaches to reduce the annotation bottleneck by making use of large-scale unlabeled data for the target task. Standard self-training mechanism randomly samples instances from the unlabeled pool to pseudo-label and augment labeled data. In this work, we propose an approach to improve self-training by incorporating uncertainty estimates of the underlying neural network leveraging recent advances in Bayesian deep learning. Specifically, we propose (i) acquisition functions to select instances from the unlabeled pool leveraging Monte Carlo (MC) Dropout, and (ii) learning mechanism leveraging model confidence for self-training. As an application, we focus on text classification on five benchmark datasets. We show our methods leveraging only 20-30 labeled samples per class for each task for training and for validation can perform within 3% of fully supervised pre-trained language models fine-tuned on thousands of labeled instances with an aggregate accuracy of 91% and improving by upto 12% over baselines.

==> impact.tex <==
\section{Broader Impact}

In this work, we introduce a framework for self-training of neural language models with only a few labeled examples. 

This work is likely to increase progress of NLP applications and drive the development of general-purpose language systems especially for domains with limited resources. While it is not only expensive to acquire large amounts of labeled data for every task and language, in many cases, we cannot perform large-scale labeling due to access constraints from privacy and compliance concerns. The latter concerns are amplified while dealing with sensitive user data for various personalization tasks and recommendation. Our framework helps in this regard for the NLP systems to obtain state-of-the-art-performance while alleviating privacy concerns. 

To this end, our framework can be used for applications in finance, legal, healthcare, retail and other domains where adoption of deep neural network has been hindered due to lack of large-scale manual annotations on user data.  

While our framework accelerates the progress of NLP, it also suffers from associated societal implications of automation ranging from job losses for workers who provide annotations as a service as well as for other industries relying on human labor. Additionally, it suffers from similar concerns as with the use of NLP models by malicious agents for propagating bias, misinformation and indulging in other nefarious activities. 

However, many of these concerns can also be alleviated with our framework to develop better detection models and mitigation strategies with only a few representative examples of such intents. 
